The Simons Observatory: Astro2020 Decadal Project Whitepaper

The Simons Observatory (SO) is a ground-based cosmic microwave background (CMB) experiment sited on Cerro Toco in the Atacama Desert in Chile that promises to provide breakthrough discoveries in fundamental physics, cosmology, and astrophysics. Supported by the Simons Foundation, the Heising-Simons Foundation, and with contributions from collaborating institutions, SO will see first light in 2021 and start a five year survey in 2022. SO has 287 collaborators from 12 countries and 53 institutions, including 85 students and 90 postdocs. The SO experiment in its currently funded form ('SO-Nominal') consists of three 0.4 m Small Aperture Telescopes (SATs) and one 6 m Large Aperture Telescope (LAT). Optimized for minimizing systematic errors in polarization measurements at large angular scales, the SATs will perform a deep, degree-scale survey of 10% of the sky to search for the signature of primordial gravitational waves. The LAT will survey 40% of the sky with arc-minute resolution. These observations will measure (or limit) the sum of neutrino masses, search for light relics, measure the early behavior of Dark Energy, and refine our understanding of the intergalactic medium, clusters and the role of feedback in galaxy formation. With up to ten times the sensitivity and five times the angular resolution of the Planck satellite, and roughly an order of magnitude increase in mapping speed over currently operating ("Stage 3") experiments, SO will measure the CMB temperature and polarization fluctuations to exquisite precision in six frequency bands from 27 to 280 GHz. SO will rapidly advance CMB science while informing the design of future observatories such as CMB-S4.

==> address_bac.tex <==
\noindent
{\scriptsize
{$^{2}$~University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK}\\
{$^{3}$~Department of Physics, Faculty of Science, Kyoto University, Kyoto 606, Japan}\\
{$^{4}$~School of Physics and Astronomy, Cardiff University, The Parade, Cardiff, CF24 3AA, UK}\\
{$^{5}$~Department of Physics and Astronomy, University of Pennsylvania, 209 South 33rd Street, Philadelphia, PA, USA 19104}\\
{$^{6}$~Kavli Institute for Particle Astrophysics and Cosmology, Menlo Park, CA 94025}\\
{$^{7}$~SLAC National Accelerator Laboratory, Menlo Park, CA 94025}\\
{$^{8}$~Center for Computational Astrophysics, Flatiron Institute, 162 5th Avenue, New York, NY 10010, USA}\\
{$^{9}$~Department of Physics, University of California, Berkeley, CA, USA 94720}\\
{$^{10}$~Department of Physics, Stanford University, Stanford, CA 94305}\\
{$^{11}$~Computational Cosmology Center, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}\\
{$^{12}$~Department of Physics, University of California San Diego, CA, 92093 USA}\\
{$^{13}$~Physics Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, USA}\\
{$^{14}$~Kavli Institute for The Physics and Mathematics of The Universe (WPI), The University of Tokyo, Kashiwa, 277- 8583, Japan}\\
{$^{15}$~NIST Quantum Sensors Group, 325 Broadway Mailcode  687.08, Boulder, CO, USA 80305}\\
{$^{16}$~Department of Physics and Astronomy, Rutgers,  The State University of New Jersey, Piscataway, NJ USA 08854-8019}\\
{$^{17}$~International School for Advanced Studies (SISSA), Via Bonomea 265, 34136, Trieste, Italy}\\
{$^{18}$~INFN, Sezione di Trieste, Padriciano, 99, 34149 Trieste, Italy}\\
{$^{19}$~Department of Physics, University of Michigan, Ann Arbor, USA 48103}\\
{$^{20}$~Kavli Institute for Cosmology Cambridge, Madingley Road, Cambridge CB3 0HA, UK}\\
{$^{21}$~Institute of Astronomy, Madingley Road, Cambridge CB3 0HA, UK}\\
{$^{22}$~Department of Physics and Astronomy, University of New Mexico, Albuquerque, NM 87131, USA}\\
{$^{23}$~AstroParticule et Cosmologie, Univ Paris Diderot, CNRS/IN2P3, CEA/Irfu, Obs de Paris, Sorbonne Paris Cit\'e, France}\\
{$^{24}$~Department of Astronomy, Cornell University, Ithaca, NY, USA 14853}\\
{$^{25}$~Jodrell Bank Centre for Astrophysics, School of Physics and Astronomy, University of Manchester, Manchester, UK}\\
{$^{26}$~Joseph Henry Laboratories of Physics, Jadwin Hall, Princeton University, Princeton, NJ, USA 08544}\\
{$^{27}$~DAMTP, Centre for Mathematical Sciences, University of Cambridge, Wilberforce Road, Cambridge CB3 OWA, UK}\\
{$^{28}$~School of Physics, University of Melbourne, Parkville, VIC 3010, Australia}\\
{$^{29}$~Instituto de Astrof\'isica and Centro de Astro-Ingenier\'ia, Facultad de F\`isica, Pontificia Universidad Cat\'olica de Chile, Av. Vicu\~na Mackenna 4860, 7820436 Macul, Santiago, Chile}\\
{$^{30}$~Canadian Institute for Theoretical Astrophysics, University of Toronto, 60 St.~George St., Toronto, ON M5S 3H8, Canada}\\
{$^{31}$~School of Electrical, Computer, and Energy Engineering, Arizona State University, Tempe, AZ USA}\\
{$^{32}$~Department of Physics \& Astronomy, University of Sussex, Brighton BN1 9QH, UK}\\
{$^{33}$~Department of Physics, York University, 157, 161 Campus Walk, North York, ON}\\
{$^{34}$~Department of Physics, Cornell University, Ithaca, NY, USA 14853}\\
{$^{35}$~Institute for Advanced Study, 1 Einstein Dr, Princeton, NJ 08540}\\
{$^{36}$~Imperial College London, Blackett Laboratory, SW7 2AZ UK}\\
{$^{37}$~Department of Applied and Engineering Physics, Cornell University, Ithaca, NY, USA 14853}\\
{$^{38}$~Astrophysics and Cosmology Research Unit, School of Mathematics, Statistics and Computer Science, University of KwaZulu-Natal, Durban 4041, South Africa}\\
{$^{39}$~Physics Department, McGill University, Montreal, QC H3A 0G4, Canada}\\
{$^{40}$~The Oskar Klein Centre for Cosmoparticle Physics, Department of Physics, Stockholm University, AlbaNova, SE-106 91 Stockholm, Sweden}\\
{$^{41}$~Department of Astrophysical Sciences, Peyton Hall,  Princeton University, Princeton, NJ,  USA 08544}\\
{$^{42}$~Institut d'Astrophysique Spatiale, CNRS (UMR 8617), Univ. Paris-Sud, Universit\'{e} Paris-Saclay, B\^{a}t. 121, 91405 Orsay, France.}\\
{$^{43}$~Berkeley Center for Cosmological Physics, University of California, Berkeley, CA 94720, USA}\\
{$^{44}$~Simon Fraser University, 8888 University Dr, Burnaby, BC V5A 1S6, Canada}\\
{$^{45}$~Department of Physics, Florida State University, Tallahassee FL, USA 32306}\\
{$^{46}$~Department of Physics, University of Florida, Gainesville, Florida 32611, USA}\\
{$^{47}$~School of Earth and Space Exploration, Arizona State University, Tempe, AZ, USA 85287}\\
{$^{48}$~University of Arizona, 933 N Cherry Ave, Tucson, AZ 85719}\\
{$^{49}$~Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh, PA, USA 15260}\\
{$^{50}$~Department of Physics and Astronomy, University of British Columbia, Vancouver, BC, Canada V6T 1Z1}\\
{$^{51}$~Physics and Astronomy Department, Stony Brook University, Stony Brook, NY USA 11794}\\
{$^{52}$~High Energy Accelerator Research Organization (KEK), Tsukuba, Ibaraki 305-0801, Japan}\\
{$^{53}$~Department of Astronomy and Astrophysics, The Pennsylvania State University, University Park, PA 16802}\\
{$^{54}$~Institute for Gravitation and the Cosmos, The Pennsylvania State University, University Park, PA 16802}\\
{$^{55}$~Astronomical Institute, Graduate School of Science, Tohoku University, Sendai, 980-8578, Japan}\\
{$^{56}$~McWilliams Center for Cosmology, Department of Physics, Carnegie Mellon University, 5000 Forbes Avenue, Pittsburgh, PA 15213, USA}\\
{$^{57}$~Laboratoire de l'Acc\'el\'erateur Lin\'eaire, Univ. Paris-Sud, CNRS/IN2P3, Universit\'e Paris-Saclay, Orsay, France}\\
{$^{58}$~Department of Physics, University of Rome ``La Sapienza'', Piazzale Aldo Moro 5, I-00185 Rome, Italy}\\
{$^{59}$~Department of Astronomy and Astrophysics, University of Toronto, 50 St.~George St., Toronto, ON M5S 3H4, Canada}\\
{$^{60}$~Dunlap Institute for Astronomy and Astrophysics, University of Toronto, 50 St.~George St., Toronto, ON M5S 3H4, Canada}\\
{$^{61}$~School of Physics and Astronomy, Sun Yat-Sen University, 135 Xingang Xi Road, Guangzhou, China}\\
{$^{62}$~Perimeter Institute 31 Caroline Street North, Waterloo, Ontario, Canada, N2L 2Y5}\\
{$^{63}$~Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}\\
{$^{64}$~Department of Physics, Yale University, New Haven, CT 06520, USA}\\
{$^{65}$~University of Southern California. Department of Physics and Astronomy, 825 Bloom Walk ACB 439, Los Angeles, CA 90089-0484}\\
{$^{66}$~Van Swinderen Institute for Particle Physics and Gravity, University of Groningen, Nijenborgh 4, 9747 AG Groningen, The Netherlands}\\
{$^{67}$~Kapteyn Astronomical Institute, University of Groningen, P.O. Box 800, 9700 AV Groningen, The Netherlands}\\
{$^{68}$~Dedman College of Humanities and Sciences, Department of Physics, Southern Methodist University, 3215 Daniel Ave. Dallas, Texas 75275-0175}\\
{$^{69}$~Milan University, Via Festa del Perdono, 7, 20122 Milano MI, Italy}\\
{$^{70}$~University of Ferrara, Via Savonarola, 9, 44121 Ferrara FE, Italy}\\
{$^{71}$~Department of Physics and Astronomy, Haverford College,Haverford, PA, USA 19041}\\
{$^{72}$~Raymond and Beverly Sackler School of Physics and Astronomy, Tel Aviv University, P.O. Box 39040, Tel Aviv 6997801, Israel}\\
{$^{73}$~Department of Physics and Engineering, 720 S. Church St., West Chester, PA 19383}\\
{$^{74}$~Department of Physics and Astronomy, University of California Los Angeles, 475 Portola Plaza, Los Angeles, CA 9009}\\
{$^{75}$~NASA/Goddard Space Flight Center, Greenbelt, MD, USA 20771}
}

==> authors_bac.tex <==
%Jo edited this file from Renee's auto-version! Will fix for future versions.

% DO NOT EDIT THIS FILE. EDITS WILL BE OVERWRITTEN.
% AUTO-GENERATED WITH make-iop-author-list.py
% FROM authors.txt AND affils.txt
The~Simons~Observatory~Collaboration:
Max~Abitbol$^{2}$,
Shunsuke~Adachi$^{3}$,
Peter~Ade$^{4}$,
James~Aguirre$^{5}$,
Zeeshan~Ahmed$^{6,7}$,
Simone~Aiola$^{8}$,
Aamir~Ali$^{9}$,
Steve~Allen$^{10,7}$,
David~Alonso$^{2}$,
Marcelo~A.~Alvarez$^{9,11}$,
Kam~Arnold$^{12}$,
Peter~Ashton$^{9,13,14}$,
Jason~Austermann$^{15}$,
Humna~Awan$^{16}$,
Carlo~Baccigalupi$^{17,18}$,
Taylor~Baildon$^{19}$,
Anton~Baleato~Lizancos$^{20,21}$,
Darcy~Barron$^{22}$,
James~Bartlett$^{23}$,
Nick~Battaglia$^{24,8}$,
Richard~Battye$^{25}$,
Eric~Baxter$^{5}$,
Andrew~Bazarko$^{26}$,
James~A.~Beall$^{15}$,
Rachel~Bean$^{24}$,
Dominic~Beck$^{23}$,
Shawn~Beckman$^{9}$,
Benjamin~Beringue$^{27}$,
Federico~Bianchini$^{28}$,
Steven~Boada$^{16}$,
David~Boettger$^{29}$,
Boris~Boillet$^{25}$,
J.~Richard~Bond$^{30}$,
Julian~Borrill$^{11,9}$,
Michael~L.~Brown$^{25}$,
Sarah~Marie~Bruno$^{26}$,
Sean~Bryan$^{31}$,
Erminia~Calabrese$^{4}$,
Victoria~Calafut$^{24}$,
Paolo~Calisse$^{12,29}$,
Julien~Carron$^{32}$,
Juan~Cayuso$^{33}$,
Anthony~Challinor$^{20,27,21}$,
Grace~Chesmore$^{19}$,
Yuji~Chinone$^{9,14}$,
Jens~Chluba$^{25}$,
Hsiao-Mei~Sherry~Cho$^{6,7}$,
Steve~Choi$^{34}$,
Phillip~Clark$^{20,27}$,
Susan~Clark$^{26,35}$,
Carlo~Contaldi$^{36}$,
Gabriele~Coppi$^{5}$,
Nicholas~F.~Cothard$^{37}$,
Kevin~Coughlin$^{19}$,
Will~Coulton$^{20,27}$,
Devin~Crichton$^{38}$,
Kevin~D.~Crowley$^{12}$,
Kevin~T.~Crowley$^{26}$,
Ari~Cukierman$^{6,10,9}$,
John~M.~D'Ewart$^{7}$,
Rolando~D\"{u}nner$^{29}$,
Tijmen~de~Haan$^{13,9}$,
Mark~Devlin$^{5}$,
Simon~Dicker$^{5}$,
Matt~Dobbs$^{39}$,
Bradley~Dober$^{15}$,
Cody~J.~Duell$^{34}$,
Shannon~Duff$^{15}$,
Adri~Duivenvoorden$^{40}$,
Jo~Dunkley$^{26,41}$,
Hamza~El~Bouhargani$^{23}$,
Josquin~Errard$^{23}$,
Giulio~Fabbian$^{42}$,
Stephen~Feeney$^{8}$,
James~Ferguson$^{20,27}$,
Simone~Ferraro$^{43}$,
Raphael~Flauger$^{12}$,
Pedro~Flux\`a$^{29}$,
Katherine~Freese$^{19,40}$,
Josef~C.~Frisch$^{6}$,
Andrei~Frolov$^{44}$,
George~Fuller$^{12}$,
Brittany~Fuzia$^{45}$,
Nicholas~Galitzki$^{12}$,
Patricio~A.~Gallardo$^{34}$,
Jose~Tomas~Galvez~Ghersi$^{44}$,
Ken~Ganga$^{23}$,
Jiansong~Gao$^{15}$,
Eric~Gawiser$^{16}$,
Martina~Gerbino$^{40}$,
Vera~Gluscevic$^{35,26,46}$,
Neil~Goeckner-Wald$^{9}$,
Joseph~Golec$^{19}$,
Sam~Gordon$^{47}$,
Megan~Gralla$^{48}$,
Daniel~Green$^{12}$,
Arpi~Grigorian$^{15}$,
John~Groh$^{9}$,
Chris~Groppi$^{47}$,
Yilun~Guan$^{49}$,
Jon~E.~Gudmundsson$^{40}$,
Mark~Halpern$^{50}$,
Dongwon~Han$^{51}$,
Peter~Hargrave$^{4}$,
Katie~Harrington$^{19}$,
Masaya~Hasegawa$^{52}$,
Matthew~Hasselfield$^{53,54}$,
Makoto~Hattori$^{55}$,
Victor~Haynes$^{25}$,
Masashi~Hazumi$^{52,14}$,
Yizhou~He$^{56}$,
Erin~Healy$^{26}$,
Shawn~W.~Henderson$^{6,7}$,
Sophie~Henrot-Versille$^{57}$,
Brandon~Hensley$^{41}$,
Carlos~Hervias-Caimapo$^{25}$,
Charles~A.~Hill$^{9,13}$,
J.~Colin~Hill$^{8,35}$,
Gene~Hilton$^{15}$,
Matt~Hilton$^{38}$,
Adam~D.~Hincks$^{58,30}$,
Gary~Hinshaw$^{50}$,
Ren\'ee~Hlo\v{z}ek$^{59,60}$,
Shirley~Ho$^{13}$,
Shuay-Pwu~Patty~Ho$^{26}$,
Logan~Howe$^{12}$,
Zhiqi~Huang$^{61}$,
Johannes~Hubmayr$^{15}$,
Kevin~Huffenberger$^{45}$,
John~P.~Hughes$^{16}$,
Anna~Ijjas$^{26}$,
Margaret~Ikape$^{59,60}$,
Kent~Irwin$^{6,10,7}$,
Andrew~H.~Jaffe$^{36}$,
Bhuvnesh~Jain$^{5}$,
Oliver~Jeong$^{9}$,
Matthew~Johnson$^{62,33}$,
Baptiste~Jost$^{23}$,
Daisuke~Kaneko$^{14}$,
Ethan~D.~Karpel$^{6,10}$,
Nobuhiko~Katayama$^{14}$,
Brian~Keating$^{12}$,
Reijo~Keskitalo$^{11,9}$,
Theodore~Kisner$^{11,9}$,
Kenji~Kiuchi$^{63}$,
Jeff~Klein$^{5}$,
Kenda~Knowles$^{38}$,
Brian~Koopman$^{64}$,
Arthur~Kosowsky$^{49}$,
Nicoletta~Krachmalnicoff$^{17}$,
Chao-Lin~Kuo$^{6,10,7}$,
Akito~Kusaka$^{13,63}$,
Phil~LaPlante$^{5}$,
Jacob~Lashner$^{65}$,
Adrian~Lee$^{9,13}$,
Eunseong~Lee$^{25}$,
David~Leon$^{12}$,
Antony~Lewis$^{32}$,
Yaqiong~Li$^{26}$,
Zack~Li$^{41}$,
Michele~Limon$^{5}$,
Eric~Linder$^{13,9}$,
Jia~Liu$^{41}$,
Carlos~Lopez-Caraballo$^{29}$,
Thibaut~Louis$^{57}$,
Lindsay~Lowry$^{12}$,
Marius~Lungu$^{26}$,
Mathew~Madhavacheril$^{41}$,
Daisy~Mak$^{36}$,
Felipe~Maldonado$^{45}$,
Hamdi~Mani$^{47}$,
Ben~Mates$^{15}$,
Frederick~Matsuda$^{14}$,
Lo\"ic~Maurin$^{29}$,
Phil~Mauskopf$^{47}$,
Andrew~May$^{25}$,
Nialh~McCallum$^{25}$,
Chris~McKenney$^{15}$,
Jeff~McMahon$^{19}$,
P.~Daniel~Meerburg$^{20,27,21,66,67}$,
Jean~-Baptiste~Melin$^{23}$,
James~Mertens$^{62}$,
Joel~Meyers$^{30,68}$,
Amber~Miller$^{65}$,
Mark~Mirmelstein$^{32}$,
Kavilan~Moodley$^{38}$,
Moritz~Munchmeyer$^{62}$,
Charles~Munson$^{19}$,
Masaaki~Murata$^{63}$,
Sigurd~Naess$^{8}$,
Toshiya~Namikawa$^{20,27}$,
Federico~Nati$^{69}$,
Martin~Navaroli$^{12}$,
Laura~Newburgh$^{64}$,
Ho~Nam~Nguyen$^{51}$,
Andrina~Nicola$^{26}$,
Mike~Niemack$^{34}$,
Haruki~Nishino$^{63}$,
Yume~Nishinomiya$^{63}$,
John~Orlowski-Scherer$^{5}$,
Luca~Pagano$^{70}$,
Lyman~Page$^{26}$,
Bruce~Partridge$^{71}$,
Francesca~Perrotta$^{17}$,
Phumlani~Phakathi$^{38}$,
Lucio~Piccirillo$^{25}$,
Elena~Pierpaoli$^{12}$,
Giampaolo~Pisano$^{4}$,
Davide~Poletti$^{17}$,
Heather~Prince$^{41}$,
Roberto~Puddu$^{29}$,
Giuseppe~Puglisi$^{6,10}$,
Srinivasan~Raghunathan$^{28}$,
Chris~Raum$^{9}$,
Christian~L.~Reichardt$^{28}$,
Mathieu~Remazeilles$^{25}$,
Yoel~Rephaeli$^{72}$,
Dominik~Riechers$^{24}$,
Naomi~Robertson$^{26}$,
Felipe~Rojas$^{29}$,
Aditya~Rotti$^{25}$,
Anirban~Roy$^{17}$,
Sharon~Sadeh$^{72}$,
Yuki~Sakurai$^{14}$,
Maria~Salatino$^{23}$,
Mayuri~Sathyanarayana~Rao$^{9,13}$,
Lauren~Saunders$^{64}$,
Emmanuel~Schaan$^{13}$,
Marcel~Schmittfull$^{35}$,
Neelima~Sehgal$^{51}$,
Joseph~Seibert$^{12}$,
Uros~Seljak$^{9,13}$,
Paul~Shellard$^{20,27}$,
Blake~Sherwin$^{20,27}$,
Meir~Shimon$^{72}$,
Carlos~Sierra$^{19}$,
Jonathan~Sievers$^{38}$,
Cristobal~Sifon$^{41}$,
Precious~Sikhosana$^{38}$,
Maximiliano~Silva-Feaver$^{12}$,
Sara~M.~Simon$^{19}$,
Adrian~Sinclair$^{47}$,
Praween~Siritanasak$^{12}$,
Kendrick~Smith$^{62}$,
Wuhyun~Sohn$^{20,27}$,
David~Spergel$^{8,41}$,
Suzanne~T.~Staggs$^{26}$,
George~Stein$^{30,59}$,
Jason~R.~Stevens$^{34}$,
Radek~Stompor$^{23}$,
Aritoki~Suzuki$^{13}$,
Osamu~Tajima$^{3}$,
Satoru~Takakura$^{14}$,
Grant~Teply$^{12}$,
Daniel~B.~Thomas$^{25}$,
Ben~Thorne$^{41,2}$,
Robert~Thornton$^{73}$,
Hy~Trac$^{56}$,
Jesse~Treu$^{26}$,
Mathieu~Tristram$^{57}$,
Calvin~Tsai$^{12}$,
Carole~Tucker$^{4}$,
Joel~Ullom$^{15}$,
Sunny~Vagnozzi$^{40}$,
Alexander~van~Engelen$^{30}$,
Jeff~Van~Lanen$^{15}$,
Daniel~D.~Van~Winkle$^{7}$,
Eve~M.~Vavagiakis$^{34}$,
Clara~Verg\`es$^{23}$,
Michael~Vissers$^{15}$,
Kasey~Wagoner$^{26}$,
Samantha~Walker$^{15}$,
Jon~Ward$^{5}$,
Ben~Westbrook$^{9}$,
Caleb~Wheeler$^{47}$,
Nathan~Whitehorn$^{74}$,
Jason~Williams$^{65}$,
Joel~Williams$^{25}$,
Ed~Wollack$^{75}$,
Zhilei~Xu$^{5}$,
Siavash~Yasini$^{12}$,
Edward~Young$^{6,10}$,
Byeonghee~Yu$^{9}$,
Cyndia~Yu$^{6,10}$,
Fernando~Zago$^{49}$,
Mario~Zannoni$^{69}$,
Hezi~Zhang$^{49}$,
Ningfeng~Zhu$^{5}$
and
Andrea~Zonca$^{12}$



==> expt_bac.tex <==


%\subsection{Requirements Flowdown}

%The SO science forecasts are based on two sensitivity models: ``baseline'' and ``goal.'' These models include instrumental noise based on a detailed experimental model \cite{bolocalc}, empirical atmospheric noise, and the impact of the finite resolution of the beam sizes.   The instrumental perimeters (e.g., detector yield, optical efficiency, and detector loading) used in determining these noise forecasts are pessimistic relative to achieved performance in previous experiments.   For reference, the detector array sensitivity predicted for the baseline (goal) model is 60\% (30\%) worse compared to the on sky performance of the nearly identical AdvACT detector arrays \cite{choi}.  These noise models are conservative to account for the risks associated with a project of this scale.

%These models produce  noise curves ($N_\ell$) for each of the six SO frequency bands which are presented in Figure XXX of \cite{SO_forecast_paper}.  The baseline model represents the instrumental requirements for the noise of SO. Systematic effects are required to be sub-dominant to these levels.   



%The baseline and goal models were determined after an extensive suite of trade studies of alternative telescope and receiver configurations.  This optimization resulted in the choice of a 6 m diameter large aperture telescope (LAT), and three 0.44 m small aperture telescopes (SATs). The two aperture sizes were required to achieve sensitivity and control of systematic effects over a range of angular scales that extends from $\sim 10^\circ$ to $1'$ scale.  

%The size of the large aperture telescope was chosen to maximize the science return of SO with respect to lensing and the high-$\ell$ CMB while balancing the cluster science goals against cost.  The large optical throughput telescope design \cite{niemack} was required to field the large number of pixels needed to meet our sensitivity targets and to enable future expansion.  This large filed of view will be populated up to 13 independent optics tubes (cameras), each with just over an octave of bandwidth.  This bandwidth is compatible with available optical components (anti-reflection (AR) coated lenses and filters) and established dichroic CMB polarimeter designs \cite{horn,sinuous}.

%The small aperture telescope design was chosen to be a 0.44 m refracting telescope in order to: (1) enable the implementation of a half-wave plate polarization modulator to mitigate atmospheric noise and systematic effects; (2) enable reliable compact cryogenic  and room-temperature baffling, and (3) enable the use of silicon lenses with robust and proven anti-reflection coatings.  An array of three telescopes was chosen to realize the required sensitivity and top cover the required frequency range using the same octave bandwidth technologies used for the LAT.

%The six SO bands were chosen to be compatible with the available atmospheric windows and grouped into three types of dicrhoic detectors: low frequency (LF), mid frequency (MF) and ultra high frequency (UHF) which cover the 28 and 40, the 90 and 150, and the 220 and 280 GHz bands, respectively.  The balance of cameras at each frequency was determined by optimizing the science return of the SATs and LAT subject to the constraint of fixed cost.  This resulted in a configuration of 1 LF, 4 MF, and 2 UHF optics tubes on the LAT; and 2 MF and 1 UHF SATs with a LF SAT deployed in place of a MF for a subset of our observations.

%The scientific optimization of the scan strategy resulted in independent SAT and LAT surveys since the SAT survey does not require delensing to achieve our science goals.  Therefore the SAT survey is chosen to limit sky area to the best foreground regions while retaining the ability to verify any detection of $r$ by testing isotropy across different patches.  The LAT survey is designed to maximize its area to return the best possible constraints on the primary CMB, lensing, clusters, and enable significant cross-correlations with nearly all the upcoming optical, X-ray, and radio surveys.  The SAT and LAT surveys are presented in Figure \ref{fig:survey}

%\textbf{(Jeff, 0.75 page)}

\section{Technical Overview}
\label{sec:experiment}
The SO builds on technology and analysis techniques developed and proven by the CMB community over the last several decades.  As with previous generations, the SO has made incremental improvements based on lessons learned.  For example, the %exact
designs of the cryogenic optical components have been fine-tuned to optimize performance and minimize potential systematic effects.  
The massive scaling of the project, with 5x more detectors than have ever been deployed for CMB, has required targeted significant development in %the area of 
detector multiplexing (Technology Driver, \S\ref{sec:detectors}).
% which is now complete (Technolgy. 
Now in its implementation phase, the SO has retired most of the technical risks.  We are moving forward with a significant analysis pipeline design which addresses the scaling challenges associated with the large number of detectors and larger sky coverage.

The SO site at Cerro Toco is well established: CMB experiments have been operating there since 1998.  The site is near one of the largest mining centers in the world which offers a wide range of logistical advantages that reduce cost and risk.
%, dramatically reducing the cost and risk of complex efforts like SO.  
These include year-round access via commercial airline in 1-2 days from North America, readily available commercial housing, a local skilled workforce, major construction equipment, and high-bandwidth internet allowing full data transfer and remote operation.

\red{Need to specify essential performance parameters: in Sec 2 add couple sentences on noise levels and angular resolution need to reach, and systematics minimization, and link to it here.}

%\begin{figure}[tbc]
 %   \centering
  %  \includegraphics[width=5 in]{figs/sat_photos.png}
%\caption{\small The Small Aperture Telescopes (SATs): design and fabrication of parts in progress. (a) CAD drawing of a SAT on its three-axis rotation platform, (b) the SAT cryostat CAD rendering, (c) one of the actual cryostats with completed fabrication and vacuum validation, (d) the rotation mechanism of one of the 55-cm-diameter cryogenic half-wave plates, and (e) an aluminum 1-K optics tube housing with 70-cm outer diameter.}
%under CMM inspection.\red{polish text}}
%    \label{fig:SAT}
%\end{figure}

\vspace{-.1in}
\subsection{Small Aperture Telescopes\label{sec:SAT}}
The three SATs, each with a single optics tube, will together contain 30,000 detectors operating at 100~mK. They adopt a design highly optimized for measuring the polarization of the CMB at degree scales (Fig. \ref{fig:Instrument}). Each SAT optics tube houses seven detector arrays, and will have a continuously rotating half-wave plate to modulate the large-scale atmospheric signal. Two SATs will observe at 93 and 145 GHz, one at 225 and 280 GHz; an additional low-frequency optics tube at 27 and 39 GHz will be deployed for a single year of observations. 
%We will deploy three SATs containing 30,000 detectors in total.  Two of them will be with the MF bands and one will be with the UHF bands.  An LF focal plane and optics tube will later be deployed replacing one of the MF tubes, acquiring one-year observation.  Each cryostat houses one optical chain and a focal plane of seven 15-cm detector wafers.  
%Each optics tube has a cryostat with four cryogenic stages: the 100-mK and 1-K stages are cooled by a dilution refrigerator, and the 4-K and 40-K stages are cooled by a pulse-tube cooler.

The optics system has a 42-cm stop aperture and a 35-degree diameter field of view.  This is enabled by three 46-cm diameter silicon lenses with anti-reflecting metamaterial surfaces.  The entire optical system is cooled to 1~K. 
%chain, including all the lenses and the aperture stop, is cooled down to 1-K; this leads to significant improvement over 4-K optics and the dilution refrigerator provides a significant sensitivity gain.  
An intensive ring-baffle scheme with engineered black body absorbers controls stray light.
%inside the 1-K optics-tube volume. 
A 50~cm diameter rotating 40~K sapphire half-wave plate is located near the sky side of the aperture stop.
%, on the 40-K stage.  Each consists of a wide-band multi-layer sapphire half-wave plate and the rotation mechanism has a superconducting mag-lev bearing, enabling stable operation at low temperature and a large clear diameter of 50-cm.  
This significantly mitigates instrumental systematics and rejects atmospheric fluctuations; both are crucial for the sensitivity to degree-scale polarization.

%Warm optical baffling comprises three stages: the fore baffle attached to the cryostat, co-moving shield attached to the elevation stage of the platform, and the ground screen.  
The entire SAT cryostat, fore baffle and co-moving shield, and the supporting electronics are mounted on a three-axis platform.  The platform allows fast scanning in azimuth and rotation around the line-of-sight for systematic control.
The warm baffling is an integrated part of our optics design, and the key for the control of far sidelobe and ground-synchronous systematics.  %Our design is such that the ray has to diffract at least twice to hit the ground or mountain. 

\vspace{-.2in}
\subsection{Large Aperture Telescope \label{sec:LAT}}
\begin{figure}
    \centering
    \includegraphics[height=3.4 in]{figs/Combined_Instrument_v1.JPG}
    \caption{\small The universal microwave-multiplexing module (UMM) is combined with the detector wafer to form the universal focal plane module (UFM) (with dummy silicon parts shown here).  The modules are designed such that they can be incorporated into either the Large Aperture Telescope Receiver (LATR), or the Small Aperture Telescopes (SATs).  The LATR is then installed in the Large Aperture Telescope (LAT) and the SAT is installed on the SAT Platform (SATP).}
    \label{fig:Instrument}
\end{figure}


The LAT is a 6~m diameter crossed-Dragone telescope designed with an 8$^\circ$ field of view providing roughly seven times the throughput of current Stage 3 telescopes (Fig. \ref{fig:Instrument}). The LAT is being built by Vertex Antennentechnik %in Germany 
in parallel with the CCAT-prime sub-millimeter telescope, and both are planned for installation in Chile in 2021 \citep{parshley/etal:2018}.

Designed to take advantage of the capabilities of the LAT, the LAT receiver (LATR) will be the largest cryogenic camera for CMB studies ever built.  
%Naturally, it is correspondingly larger and more complex than the previous generation of receivers such as the ones for the Atacama Cosmology Telescope and the South Pole Telescope.  
It is 2.5~m in diameter and over 2.6~m long accommodating up to 13 optics tubes.  It must cool a metric ton of material to 4 degrees above absolute zero and over 100 kg to 0.1 degrees above absolute zero.  

%With an order of magnitude more detectors than previous instruments, t
The LATR is designed to maximize sensitivity while implementing new designs to increase robustness against systematic effects.  
%Each pixel is dual-band and dual-frequency resulting in four Transition Edge Sensors (TES) per pixel.  Microwave multiplexing technology was developed by SO to read out as many as 2000 TES detectors with a single pair of coaxial cables.  The readout is controlled by FPGA-based warm RF electronics developed at SLAC.
Each of the 13 optics tubes consists of three state-of-the-art anti-reflection coated silicon lenses and an array of filters.  The optical design enhances control of stray light which could ultimately limit the sensitivity of the instrument.  Extensive modeling based on past experience had driven novel design changes to meet the new specifications.  The LATR will be deployed with 7 of the 13 optics tubes. The additional 6 tubes can be added in the field (\S\ref{sec:enhance}).

%\begin{figure}
 %\includegraphics[width=0.95\textwidth]{figs/det-slide-v2.pdf}
%\caption{\small SO readout and detector modules.  The first two photos show a UMM designed to read out 2000 TESes, while the third shows a UFM model (with dummy silicon parts).}      \label{fig:dets}
%\end{figure}

\vspace{-.2in}
\subsection{Detectors and Readout\label{sec:detectors}}

%The nominal SO design requires 5x more detectors than have ever been deployed for CMB.  This massive scaling has required significant development in the area of detector multiplexing. 

%The SO analysis pipeline design has also required significant development to address the scaling challenges associated with the large number of detectors and very large sky coverage.

%The SO is moving into its implementation phase, having retired most of its technical risks.  
%STS shortened this on 5 July 19  The previous version is appended below, commented out. 

The focal planes of each of the SO telescopes will be tiled with hexagonal universal focal-plane modules (UFMs, Fig.~\ref{fig:Instrument}) based on dichroic transition edge sensor (TES) bolometric polarimeters. Each pixel contains four bolometers:  two frequency bands in two orthogonal polarizations.  The detector arrays for SO come in three frequency configurations.  The MF (90/150 GHz) and UHF (220/270 GHz) UFMs host $\sim 2000$ bolometers each, while the LF (27/40 GHz) UFMs have $\sim 200$ each. SO will employ bolometer arrays coupled through orthomode transducers to aluminum feedhorns, and arrays coupled through dual-polarization sinuous antennas and lenslets. These two flavors of arrays are made at NIST and UCB respectively, giving the project built-in risk mitigation against schedule delays due to production hold-ups at one fabrication house.   

{\bf Technology driver:} The bolometers are read out with a microwave multiplexing scheme \citep{mates/etal:2017,dober/etal:2017} that transduces each detector's CMB signals into frequency shifts of a cryogenic resonator tuned between 4 and 8 GHz. 
Here 2000 resonators are coupled to a single transmission line so that
one UFM (or up to seven LF UFMs) is read out with a single pair of coaxial cables and a dozen pairs of lines carrying biases for the detectors and readout.  For efficient filling of the focal planes, each UFM packs the cryogenic readout components directly behind a detector array  fabricated on a  150~mm wafer.  The cryogenic readout components for a UFM are collectively called the universal microwave-multiplexing module (UMM), which includes a few dozen SQUID-based multiplexing  (mux) chips and silicon boards providing shunt resistors and series inductors for each TES, mounting, and routing of lines. Each UMM is validated as a unit, and then coupled to a detector stack comprising a detector wafer with associated optical coupling components on its sky side and back-termination components on its non-sky side. The resulting UFMs are validated three at a time in one of several 100-mK test systems using a combination of dark tests and cryogenic load tests.  

%The focal planes of each of the SO telescopes will be tiled with hexagonal universal focal-plane modules (UFMs) based on dichroic transition edge sensor (TES) bolometric polarimeters, shown in Figure~\ref{fig:dets}.  Each pixel contains four bolometers:  two frequency bands in two orthogonal polarizations.  The detector arrays for SO come in three frequency configurations and two optical-coupling configurations.  The MF (90/150 GHz) and UHF (220/270 GHz) UFMs host $\sim 2000$ bolometers each, while the LF (27/40 GHz) UFMs have $\sim 200$ each.  Half the MF and all the UHF detector arrays collect radiation through orthomode transducers (OMTs) coupled to aluminum feedhorns, while the other half of the MF and all the LF detector arrays use dual-polarization sinuous antennas coupled to silicon lenslets.  These two flavors of arrays are made at NIST and UCB respectively, giving the project built-in risk mitigation against schedule delays due to production hold-ups at one fab house.   

%{\bf Technology driver:} The bolometers are read out with a microwave multiplexing scheme \citep{mates/etal:2017,dober/etal:2017} that transduces each detector's CMB signals into frequency shifts of a cryogenic resonator tuned between 4 and 8 GHz.  Here 2000 resonators are coupled to a single transmission line so that one UFM (or up to seven LF UFMs) is read out with a single pair of coaxial cables and a dozen pairs of ``DC" lines carrying biases for the detectors and readout.  For efficient filling of the focal planes, each UFM packs the cryogenic readout components directly behind a detector array  fabricated on a  150~mm wafer.  The cryogenic readout components for a UFM are collectively called the universal microwave-multiplexing module (UMM), which includes a few dozen SQUID-based multiplexing  (mux) chips glued to a silicon carrier board (the ``DC wafer")  that routes the DC lines and provides shunt resistors and series inductors for each TES.  The 4-8 GHz comb of probe tones for interrogating the resonators travels to and through the mux chips on coplanar waveguide (CPW) connected via wire bonds.  Large openings are cut into a silicon ``RF wafer" so it can be placed on top of the DC wafer and surround the mux chips, providing CPW interconnections and ground plane continuity. The DC lines and transmission lines are carried off the silicon boards on flexible circuits to connectors on the non-sky side of the UMM.  Each UMM is validated as a unit, and then coupled to a detector stack comprising a detector wafer with associated optical coupling components on its sky side and back-termination components on its non-sky side.  The resulting UFMs are validated up to three at a time in one of several 100-mK test systems using a combination of dark tests and cryogenic load tests.  



==> main_bac.tex <==


The Simons Observatory (SO) is a ground-based cosmic microwave background (CMB) experiment sited on the side of Cerro Toco in the Atacama Desert in Chile that promises to provide breakthrough discoveries in fundamental physics, cosmology, and astrophysics. 
Supported by the Simons Foundation, the Heising-Simons Foundation, and with contributions from university partners, SO will see first light in 2021 and start a five year survey in 2022. SO has 287 collaborators from 12 countries and 53 institutions,
including 85 students and 90 postdocs.

SO consists of three 0.5~m Small Aperture Telescopes (SATs)  and one 6~m Large Aperture Telescope (LAT).   Optimized for minimizing systematic errors in polarization measurements at large angular scales,
the SATs will perform a  deep, degree-scale survey of 10\% of the sky  to search for the signature of primordial gravitational waves.
%emanating from the Big Bang epoch.  
The LAT will survey  of 40\% of the sky with arc-minute resolution.  These observations will measure (or limit) the sum of neutrino masses, search for light relics, 
%which have the potential to be Dark Matter, 
measure the early behavior of Dark Energy, and refine our understanding of the intergalactic medium, clusters and the role of feedback in galaxy formation.

With up to 10 times the sensitivity and 5 times the angular resolution of the {\it Planck} satellite, and roughly an order of magnitude increase in mapping speed over currently operating (``Stage 3") experiments, SO will measure the temperature and polarization fluctuations to exquisite precision in six frequency bands from 27 to 280 GHz. SO will rapidly advance CMB science while informing the design of future observatories such as CMB-S4. Construction of the nominal SO configuration is fully funded, and operations and data analysis are funded for part of the planned five-year observations. We will seek federal funding to complete the observations and analysis (see \S\ref{sec:funding}). 
%Many aspects of the design and forecast work from the SO have already been directly incorporated into the reference design for CMB-S4. 
The SO has a low risk and cost efficient upgrade path -- the 6~m telescope can accommodate almost twice the baseline number of detectors and the small-aperture telescopes can be duplicated at low cost.  %Progress in ground-based experimentation has greatly benefited from continuous evolution. 
%Funding of operations, analysis, and moderate expansion of the SO will rapidly advance CMB science and inform the design of future observatories such as CMB-S4.
Funding a moderate expansion of the SO will further strengthen its scientific impact.


This white paper summarizes material presented in \cite{so_forecast:2019}, which describes the science overview, and \cite{galitzki/etal:2018,gallardo/etal:2018,orlowski-scherer/etal:2018,dicker/etal:2018,zhu/etal:2018,coppi/etal:2018,hill/etal:2018} which describe the instrument design.  %These papers provide more thorough references.  

\par \noindent

%\vspace{-.2in}
%\section{Building the Simons Observatory}
%\label{sec:building}

%%{\bf Organization, Partnerships, and Current Status:} 
%Supported by the Simons Foundation, the Heising-Simons Foundation, and with contributions from university partners, SO will see first light in 2021 and start a five year survey in 2022.   
%%SO will be located in Parque Astron\’{o}mico at an altitude of 5190 meters on the side of Cerro Toco in the Atacama Desert of Northern Chile.  The high altitude, dry climate and tropical latitude combine to make it an ideal site for our science program. 
%%SO is fully funded for construction through 2022 and partially supported for operations and analysis over five years. \S\ref{sec:funding} has a cost breakdown.
%%has a promise of \$20M in observation funds over five years.
%There are 287 
%%active
%collaborators from 12 countries and 53 institutions,
%%(US, Canada, Chile, China, France, Israel, Italy, Japan, Netherlands, South Africa, Sweden, UK), 
%including 85 students and 90 postdocs.


%There are currently 85 students and 90 postdocs working as part of the SO team.  

%SO's multi-frequency temperature and polarization maps will significantly advance those of current ``Stage 3" experiments.  
%SO will deepen our understanding of fundamental physics through its improved measurements of the amplitude of primordial gravitational waves (\S\ref{sec:primordial}), number of light relativistic species (\S\ref{sec:Neff}), and the neutrino mass (\S\ref{sec:mnu}).
%It will trace the large scale projected distribution of dark matter, gas momentum and gas pressure.  SO will search for beyond standard model physics (\S\ref{sec:de}), directly probe energy injection by galaxy formation (\S\ref{sec:gf}) and determine the duration 
% and redshift
%of the epoch of reionization (\S\ref{sec:reion}). Its legacy maps will be broadly useful with applications ranging from the search for planet X in the solar system to the detection of 20,000 clusters, numerous star-forming galaxies and radio sources (\S \ref{sec:legacy}).


%The LAT and its receiver combine to provide an order of magnitude improvement over highStage 3 CMB  instruments.  The three SATs represent a significant increase in B-mode sensitivity. \red{Say why can't do it all with LAT}
%, and are relatively easy to duplicate. - Jo - said that earlier
%so the numbers can be expanded as we understand the requirements and challenges better in the coming years. 
%SO designs build on decades of experience from the entire CMB community addressing optical designs, detector fabrication, software development, and advanced cryogenics. Each of the telescopes will have bolometric cameras (\S\ref{sec:detectors}) that will
%measure temperature and polarization fluctuations at multiple frequencies. As new measurements push sensitivity limits to impressive goals, these next generation instruments must be especially mindful of systematic errors which may have been sub-dominant in existing experiments but could limit the ultimate sensitivity of future ones.

%Jo moving this part to Technical Part
%CMB experiments have been operating at the Cerro Toco site since 1998.  The site is near one of the largest mining centers in the world which offers a wide range of logistical advantages, dramatically reducing the cost and risk of complex efforts like SO.  
%These include year-round access via commercial airline in 1-2 days from North America, readily available commercial housing, a local skilled workforce, major construction equipment, and high-bandwidth internet allowing full data transfer and remote operation.
%End move

%%{\it {In its current configuration, SO will make significant progress
%represent an important step 
%%towards all the science goals identified by
%%the cosmology community for the CMB-S4 project.  
%%%As planned, SO should make significant progress towards all of CMB-S4's science goals. 
%%Because of the modular hardware design of SO, the project can be further expanded. With additional investments (\S\ref{sec:enhance}), SO could roughly double the number of detectors in the LAT and can cost-effectively duplicate the SATs. There is significant international interest in expanding SO, and international support could be combined with federal support for both construction and extended operations. JAXA's planned LiteBIRD mission will complement SO by mapping the largest angular scales in CMB polarization.}}

%In its current configuration, SO will make significant progress towards all the science goals identified by the cosmology community for ground-based CMB in the next decade.  
%Because of the modular hardware design of SO, the project can be expanded with relatively modest additional investments in instrumentation and observations. In this scenario, SO-Enhanced (described in \S\ref{sec:enhance-subsec}) could achieve the goals outlined in Table 2.

\vspace{-.2in}
\section{Key Science Goals and Objectives}
\label{sec:science}
\input science.tex


\input experiment.tex

\label{sec:enhance-subsec}

\section{Simons Observatory and Beyond\label{sec:enhance}}

\vspace{-.1in}
\subsection{Enhancing Simons Observatory: science goals and technical overview}

While the SO will significantly advance our understanding of cosmology beyond currently operating instruments, there are potential extensions that will enhance its capabilities.  Table 2 shows the potential science yield of an Enhanced Simons Observatory that has the following upgrades: (a) filling the remaining 6 optics tubes in the LAT;
(b) adding 3 additional SATs; and (c) five additional years of operations. 
%from 2022 through 2032.

%The LAT receiver is only partially filled. With additional investment, we could fill the remaining 6 optics tubes. The combination of this upgrade and 5 additional years of operation would nearly double the sensitivity of the experiment, enabling improved measurements of neutrino mass, the number of relativistic species, the growth of structure, galaxy evolution and reionization.  The combination of LiteBIRD's $\tau$ measurement and the increased sensitivity of the enhanced SO will enable a 4$\sigma$ detection of neutrino mass, even for the minimal mass (Table 2).  In its nominal mode, SO will detect 20,000 clusters at $> 5 \sigma$, for goal sensitivity. With this enhancement, it should detect 33,000.  The signal-to-noise in its lensing and kSZ maps will be improved by $\sim 70\%$, with more than 80\% of the signal-to-noise in the CMB lensing map coming from polarization measurements.  These should be free of many of the foreground systematics that may limit temperature maps. These advances will open up new avenues of cluster and lensing science, especially in combination with optical surveys. For example, 

%SO's ability to measure large-scale polarization fluctuations and probe the physics of the early universe could also be enhanced through both extending its operations and through building copies of the SATs.  T

%There is a pending proposal to the UK Science Technology Facilities Council (STFC) that could fund additional SATs.  Federal funding could also enable the construction of additional SATs and extended operations (\S\ref{sec:funding}).  

%With 3 additional SATs and 5 additional years of operation, 


 This LAT enhancement will improve the signal-to-noise in SO's lensing maps by $\sim 70\%$, with most of the signal
 %of the signal-to-noise in the CMB lensing map 
 coming from polarization measurements, expected to be free of many foreground-induced errors that may limit temperature maps (Table 2). The SZ measurements will also improve significantly. In combination with LiteBIRD's $\tau$ measurement, SO-Enhanced targets a 4$\sigma$ detection of neutrino mass, even for the minimal mass.  
 %In its nominal mode, SO will detect 20,000 clusters at $> 5 \sigma$, for goal sensitivity. With this enhancement, it should detect 33,000.  
 %The  will be improved by $\sim 70\%$, with more than 80\% 
 %of the signal-to-noise in the CMB lensing map 
 %coming from polarization measurements, expected to be free of many of the foreground-induced errors that may limit temperature maps. The SZ measurements will improve significantly. 
 %New avenues of cluster and lensing science will open up, especially in combination with optical surveys. %For example,

With the SAT enhancement, SO could achieve a $1 \sigma$ limit on $r$ of 0.001 (Table 2). This is based on our current best estimates of foregrounds. There is a strong motivation to reach this level, with certain large-field plateau inflationary models predicting $r \approx 0.003$ \citep[e.g.,][]{starobinsky:1980}.




\vspace{-.2in}
\begin{table*}[htb!]
\centering
\caption[Simons Observatory Surveys]{Enhanced SO Science 
%(filled LAT, 3 additional SATs and 5 additional years of operation)
} \small
\begin{tabular}{ l | cc}
\hline
\hline
  &  SO-Nominal (Goal) & SO-Enhanced (Goal) \\
\hline
\hline
{\bf Lensing and SZ (LAT)} &&\\
\hline
\quad Minimal neutrino mass detection ($\mnu$=0.06~eV)\textsuperscript{a}   &  3$\sigma$ &  4$\sigma$  \\

\quad Lensing  detection (polarization-only)& 160$\sigma$ (110$\sigma$)&220$\sigma$ (180$\sigma$)\\
%\quad Lensing  detection (polarization-only) &110$\sigma$&\\
\quad Number of SZ clusters  & 20000 & 33000  \\
\quad Kinematic SZ detection (DESI cross-correlation) & 190$\sigma$ & 240 \\
\quad Measurement of Optical Depth from kSZ, \sigma(\tau) \textsuperscript{b} & 0.007 & 0.003 \\
%\quad Optical depth to reionization from kSZ & \sigma(\tau)=0.007 & \sigma(\tau)=0.003 \\
\hline
{\bf Primordial polarization (SATs)}  &&\\
\hline
\quad Tensor-to-scalar  ratio &$\sigma(r)=0.002$ & $\sigma(r)=0.001$\textsuperscript{c} \\
\hline
\hline
\end{tabular}
\begin{tablenotes}
\item \textsuperscript{a} This can be derived from {\it either} CMB lensing {\it or} SZ clusters, each in combination with LSS. Here we assume a cosmic-variance optical depth measurement from LiteBIRD.
%This could be further improved with more optically-selected galaxies for cross-correlation.
\item \textsuperscript{b} This uses the kSZ induced 4-point function \cite{ferraro/smith:2018}, a new method to study patchy reionization.
\item \textsuperscript{c} The SO-nominal case projects $\sigma(r)=0.0018$ (2 s.f.) for a residual lensing power of $A_L=0.5$. For SO-Enhanced with $A_L=0.5$ we project $\sigma(r)=0.0012$; for $A_L=0.3$ we project $\sigma(r)=0.0009$. 
\end{tablenotes}
\label{tab:enhance}
\end{table*}



  

%\red{An advantage of this approach, where we build up capability over time, is that we can modify the design of subsequent expansions of our instrumentation to incorporate advances in technology.}

\subsection{Relationship to CMB-S4 \red{(Under discussion with the S4 management)}}

%{\it (old: The Simons Observatory, even in nominal form, will help enable the science goals of CMB-S4.  Its measurements of fundamental parameters are a major advance over our current knowledge.  SO's technical developments are already helping to enable the planning for the CMB-S4 observatories.  SO's highly sensitive maps of the galactic foregrounds should help inform CMB-S4's frequency coverage and sensitivity at each frequency.  SO could find that our ability to remove foregrounds saturates when we only have ground-based data. Observatories at the South Pole will provide complementary data and independent technical expertise and insights into both foregrounds and cosmology.  The combination of these facilities could potentially become part of a larger CMB-S4 project.)}


 % with suzanne and Adrisn's mods
 %{\it {The Simons Observatory will help enable the science goals of CMB-S4.  SO's measurements of fundamental parameters are a major advance over our current knowledge. SO’s technical development work has already helped enable the planning for the CMB-S4 instrumentation, which draws from shared SO designs of the crossed-Dragone LAT, the multi-tube LATR, the half-wave-plate-equipped SAT optics, and the universal focal-plane
 %modules.  SO's highly sensitive maps of the Galactic foregrounds should help inform CMB-S4's frequency coverage and sensitivity at each frequency. SO could find that our ability to remove foregrounds saturates when we only have ground-based data. CMB-S4 will thus ideally retain the ability to modify its strategies in response to the SO data. Investment in SO and its extension could be both scientifically powerful and directly advance the development of CMB-S4. Observatories at the South Pole will provide complementary data and independent technical expertise and insights into both foregrounds and cosmology. 
 %The combination of these facilities could potentially become part of a larger CMB-S4 project. These two facilities provide the basis for the CMB-S4 reference design.}}

%MArk: As CMB-S4 moves forward, SO technology development, infrastructure and analysis pipelines could be partially or fully incorporated to help enable the science goals of CMB-S4.  In the mean time, investment in SO and Enhanced-SO will dramatically accelerate accumulated advances in the field and therefore the development of CMB-S4. SO members comprise 60\% of the CMB-S4 collaboration.  There is keen interest in the SO collaboration to move SO forward as fast as possible while supporting CMB-S4 as much as possible.  We believe achieving this will require a combination of public and private investment such as what we have proposed here.

%The Simons Observatory is an important step toward the science goals of CMB-S4.  SO's measurements of fundamental parameters  will be a major advance over our current knowledge. The timing works well. As CMB-S4 moves forward, SO technology development, infrastructure and analysis pipelines could be partially or fully incorporated into it.  In the mean time, investment in SO and Enhanced-SO will dramatically accelerate accumulated advances in the field and therefore the development of CMB-S4.  SO members comprise 60\% of the CMB-S4 collaboration.  There is keen interest in the SO collaboration to move SO forward as fast as possible while supporting CMB-S4 as much as possible.   A combination of public and private investment will make this synergistic plan possible.  

The Simons Observatory is an important step toward the science goals of CMB-S4.  The timing is such that as CMB-S4 moves forward, SO technology development, infrastructure and analysis pipelines could be partially or fully incorporated into it.  In the meantime, investment in SO and SO-Enhanced will dramatically accelerate accumulated advances in the field.  In particular, SO's highly sensitive multi-wavelength maps should help inform CMB-S4's frequency coverage and mitigation of systematic uncertainties.  SO members comprise 60\% of the CMB-S4 collaboration.  There is interest in the SO collaboration to move SO forward as fast as possible while supporting CMB-S4 as much as possible.  
A combination of public and private investment will make this synergistic plan possible. 

\vspace{-.2in}
\section{Schedule and cost estimates}
\label{sec:funding}

The SO project is well into the construction phase.  The first SAT and LATR cryostats have been delivered and are undergoing cryogenic verification.  The LAT and SATs are under construction and will be complete by 2021 and 2020 respectively.  Production of the detectors and readout will begin at the end of 2019. The SO schedule has first light for the first of the three SATs at the beginning of 2021 and full operations of the observatory in 2022.  The baseline SO-Nominal goals outlined in Table \ref{tab:enhance} will be achieved during the first five years of observations from 2022 through 2027.  SO-Enhanced instrument upgrades will be phased into the SO infrastructure and will be completed by 2027.  The SO-Enhanced goals will be achieved after an additional five years of observing from 2027 through 2032: by this time SO may be operating as part of the larger CMB-S4 project.

The SO project budget is given in Table \ref{tab:budget}.  A total of \$130M in commitments have been made towards achieving the SO-Nominal goals with an additional \$20M required for observations and analysis.  All of the SO-Enhanced instrumentation will be copies of existing instrumentation with no required technology development, hence the costs are well understood. The observation and analysis cost estimates are based on 20 years of operational experience at the site in Chile as well as scaled (from ACT) estimates of the analysis effort. All costs are in FY19 dollars. 

It is possible that international support could be incorporated into the SO-Enhanced plan.  For example, there is a pending proposal to the UK Science Technology Facilities Council (STFC) that could fund up to three additional SATs. 

  

\begin{table*}[htb!]
\centering
\caption[Simons Observatory Budget]{The Simons Observatory Budget} \small
\begin{tabular}{ l | c c c}
\hline
\hline
  &  2017-2022 & 2022-2027 & 2027-2032\\
\hline
\hline
{\bf SO-Nominal} &&\\
\hline
\quad Simons Foundation Project Funding & \$65M \\

\quad Institutional Commitments (cash) & \$10M \\
\quad Institutional Commitments (reduced overhead - est.) & \$10M \\
\quad Institutional Commitments (in kind - est.) \\
\quad \quad 30 graduate students per year & \$9M & TBD & TBD\\
\quad \quad 36 postdocs per year & \$15M & TBD & TBD \\
\quad Simons Foundation - Observations/Analysis && \$20M\\
\quad Federal Support - Observations/Analysis & & {\bf \$20M} \\
\quad Federal Support - Science Community && {\bf \$5M} \\
\hline
{\bf SO-Enhanced}  &&\\
\hline
\quad Federal Support - Instrumentation & & {\bf \$50M} \\
\quad Federal Support - Observations/Analysis &&& {\bf \$50M}\\
\quad Federal Support - Science Community &&& {\bf\$5M}\\
\hline
\hline
\end{tabular}
%\begin{tablenotes}
%no notes
%\end{tablenotes}
\label{tab:budget}
\end{table*}




\clearpage
\small{


\bibliography{so}  
}




==> science_bac.tex <==



%\def\mnu{m_\nu}
%\def\neff{$N_{\rm eff}$}

\newcommand{\map}{{\sl WMAP}}
\newcommand{\planck}{{\it Planck}}
\newcommand{\wmap}{{\it WMAP}}
\newcommand{\cobe}{{\sl COBE}}
\newcommand{\ba}{\begin{eqnarray}}
\newcommand{\ea}{\end{eqnarray}}
\newcommand{\n}      {{\bf{n}}}
\newcommand{\EV}[1]  {\langle#1\rangle}
\newcommand{\lmax}   {l_{\rm max}}
\newcommand{\mmax}   {m_{\rm max}}
\newcommand{\uKsq}   {\mbox{$\mu{\rm K}^2$}}
\newcommand{\uKrs}   {\mbox{$\mu{\rm K}\sqrt{\rm s}$}}
\newcommand{\dg}     {\mbox{$^{\circ}$}}
\newcommand{\lsim}   {\mbox{$_<\atop^{\sim}$}}
\newcommand{\gsim}   {\mbox{$_>\atop^{\sim}$}}
\newcommand{\lt}     {\mbox{$<$}}
\newcommand{\gt}     {\mbox{$>$}}
\newcommand{\order}  {{\cal O}}
\newcommand{\JJ}     {{\cal J}}
\newcommand{\<}      {\langle}
\renewcommand{\>}    {\rangle}
\newcommand{\amin}   {\mbox{$^\prime\ $}}
\newcommand{\asec}   {\mbox{$^{\prime\prime}\ $}}
\newcommand{\ddeg}   {\mbox{${\rlap.}^\circ$}}

\newcommand{\ylm}[2] {{Y_{#1#2}}}
\newcommand{\ylmcc}[2]{{Y^{*}_{#1#2}}}
\newcommand{\fnlKS}  {f_{NL}^{\rm local}}
\newcommand{\fnleq}  {f_{NL}^{\rm equil}}

\newcommand  \cm     {{\rm \,cm}}
\newcommand  \gtsim  {\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}
\newcommand  \ltsim  {\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
\newcommand{\lap} {$\stackrel{<}{_\sim}$}
\newcommand{\gap} {$\stackrel{>}{_\sim}$}

\newcommand{\LCDM}   {$\Lambda$CDM}
\newcommand{\etal}   {{\it et.al.}}

% --Equations
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\mat}[1]{\ensuremath{\mathbf #1}}
\newcommand{\neff}  {$N_{\rm eff}$}
\newcommand{\mnu} {\Sigma m_\nu}

\def\taua{\mbox{Tau A}}

\newcommand{\iras}{{\sl IRAS}}
\newcommand{\firas}{{\sl FIRAS}}
\newcommand{\cobedirbe}{{\sl COBE/DIRBE}}
\newcommand{\cobedmr}{{\sl COBE/DMR}}
\newcommand{\cobefiras}{{\sl COBE/FIRAS}}
\newcommand{\so}{SO}
\newcommand{\sa}{Simons Array}
\newcommand{\pbear}{\textsc{Polarbear}}
\newcommand{\pb}{\textsc{Polarbear}}
\newcommand{\Pb}{\textsc{Polarbear}}
\newcommand{\polarbear}{\textsc{Polarbear}}
\newcommand{\act}{ACT}
\newcommand{\mrvol}[1]{\textcolor{blue}{In charge: #1}}
\newcommand{\todo}[1]{{\bf TODO: #1}}

%Observations of the CMB have become one of the pillars of modern cosmology.  Measurements of the primary CMB provide insights into the physical processes of the early universe that contain signatures of its first moments and contain the seed for the formation of galaxies and large scale structure. 


\begin{figure}[t!]
\vspace{-.1in}
\includegraphics[width=6in]{figs/scan.pdf}
\centering
\includegraphics[width=4.3in]{figs/so_spectra_v4.pdf}
\caption{\small (Top) Planned sky coverage of the Small Aperture Telescopes (SATs, left) and Large Aperture Telescope (LAT, right, targeting maximal overlap with LSST and DESI) in Equatorial coordinates.%, overlaid on a map of Galactic dust emission. %For the SATs we anticipate a non-uniform coverage. 
%We expect to cover 40\% of the sky with the LAT, 
%avoiding observations where the Galactic emission is high (red), and
%targeting maximal overlap with LSST and DESI. 
\quad(Bottom) CMB temperature and polarization angular power spectra, showing projected SO errors compared to current data from {\it Planck} \citep{planck_overview:2018} and the BICEP/Keck array \citep{bk:2018}, and projected errors for the LiteBIRD satellite. Other current ground-based data are in Fig.~18 of \cite{planck_overview:2018}. SO will increase angular resolution compared to {\it Planck}, and will improve the sensitivity of the divergence-like E-mode and curl-like B-mode polarization signals. Other key SO statistics include the CMB lensing power spectrum, the bispectrum, the kinematic Sunyaev-Zel'dovich effect, and the number of clusters seen via the thermal Sunyaev-Zel'dovich effect.}%The precise coverage will be refined with scanning simulations.}
\label{fig:coverage}
\end{figure}


%\begin{figure}[t!]
%\centering
%%\vspace{-.2in}

%\includegraphics[width=4in]{figs/so_spectra_v4.pdf}
%\vspace{-.2in}
%\caption{\small CMB temperature and polarization angular power spectra, showing projected Simons Observatory uncertainties compared to current data from the {\it Planck} satellite \citep{planck_overview:2018} and the BICEP/Keck array \citep{bk:2018}, and projected errors for the LiteBIRD satellite. A compilation of data from other current ground-based experiments is in Fig.~18 of \citet{planck_overview:2018}. SO's Large Aperture Telescope will increase the angular resolution compared to {\it Planck}, and both the LAT and SATs will improve the sensitivity of the divergence-like E-mode and curl-like B-mode polarization signals. We will also use the SO maps to extract the CMB lensing power spectrum, the bispectrum, the kinematic Sunyaev-Zel'dovich effect, and the number of clusters seen via the thermal Sunyaev-Zel'dovich effect.}
%AK: Does this include FG uncertainty at $\ell > 3000$?.
%\label{fig:spectra}
%\end{figure}




%SO will make significant progress towards all the science goals identified by the cosmology community for ground-based CMB in the next decade.  
\vskip -0.1in
Table~\ref{tab:goals} shows our key science targets for both `baseline' and  `goal' noise levels for the SATs and LAT, described in \cite{so_forecast:2019}.
%Here we describe the science goals of the nominal SO surveys (SO-Nominal), 
The anticipated sky coverage and CMB power spectrum uncertainties are shown in Fig.~\ref{fig:coverage}.
%and the expected  in Fig. \ref{fig:spectra}. 
In the following we quote projections for baseline noise levels, which include an additional 25\% inflation factor as a proxy for additional systematic errors.  Goal noise projections are shown in parentheses. Relevant Astro2020 Science White Papers (SWP) are indicated.
%For the baseline case, we show the forecast uncertainty inflated by 25\% as a proxy for additional systematic errors. This reflects the impact of effects including, for example, beam uncertainty as described in Sec. \ref{ssec:neff}, or bandpass uncertainty \cite{Ward2018}. 

%For each science target we also give the current uncertainty, and specify which method is used. A key describing the methods is given in Table~\ref{tab:method}. In the following we describe each science target, focusing on the nominal baseline noise levels. \\


\begin{table*}[ht!]
\centering
\caption[Simons Observatory Surveys]{Summary of SO key science goals\textsuperscript{a}} \small
\begin{tabular}{ l |c| c  c|l|l}
\hline
\hline
  & Current\textsuperscript{b} & \multicolumn{2}{|c|}{ SO-Nominal (2022-27)} & Method\textsuperscript{d} & SWP \\
    &  & Baseline & Goal & & \\
%&&2022-27&2022-27&2022-32&2022-32&\\
\hline
\hline
{\bf Primordial}  &&&&&\\
{\bf \quad perturbations} (\S\ref{sec:primordial})   &&&&&\\
%{\bf  perturbations} (\S\ref{sec:primordial})  &&&&&\\
\hline
$r$ ($A_L=0.5$) & $0.03$ & $0.003$ & $0.002$\textsuperscript{e} & BB + external delensing & \cite{shandera/etal:2019} \\
$n_s$ & 0.004 & 0.002 & 0.002 &  TT/TE/EE &\cite{shandera/etal:2019} \\
 $e^{-2\tau}\mathcal{P}(k=0.2 \rm{/Mpc})$ & 3\% & 0.5\% & 0.4\% & TT/TE/EE & \cite{slosar/etal:2019b}\\
$f^{\rm local}_{\rm{NL}}$&  5&  3$ & 1 & $\kappa \kappa$ $\times$ LSST-LSS & \cite{meerburg/etal:2019}\\
&& 2 & 1 &kSZ + LSST-LSS  &\\
%&&&& &\\
\hline
{\bf Relativistic species} (\S\ref{sec:Neff}) &&&&&\\
\hline
\neff\ &  0.2 & $0.07$ & 0.05  & TT/TE/EE + $\kappa \kappa$ & \cite{green/etal:2019}\\
%&&&&&\\
\hline
{\bf Neutrino mass} (\S\ref{sec:mnu})&&&&&\\
\hline
$\mnu$ (eV, $\sigma(\tau)=0.01$) & 0.1 &  0.04 & 0.03 & $\kappa \kappa$ + DESI-BAO & \cite{dvorkin/etal:2019} \\
&& 0.04$ & 0.03 &  tSZ-N $\times$ LSST-WL &\\
%&& 0.05$ & 0.04 & tSZ-Y + DESI-BAO &\\
&&&&&\\
$\mnu$ (eV, $\sigma(\tau)=0.002$) & &   0.03$\textsuperscript{f}  & 0.02  & $\kappa \kappa$ + DESI-BAO + LB &\\
 & &   0.03  & $0.02$  &  tSZ-N $\times$ LSST-WL + LB & \\
% & &  0.04  & $0.03$  &  tSZ-Y + DESI-BAO + LB &\\
%&&&&\\
\hline
{\bf Beyond standard } &&&&&\\
{\bf \quad model} (\S\ref{sec:de}) &&&&&\\
\hline
$\sigma_8(z=1-2)$& 7\%& 2\% & 1\% &$\kappa \kappa$ + LSST-LSS & \cite{slosar/etal:2019}\\
&& 2\% & 1\% & tSZ-N $\times$ LSST-WL & \\
$H_0$ ($\Lambda$CDM) & 0.5 & 0.4 & 0.3 & TT/TE/EE + $\kappa \kappa$ & \cite{beaton/etal:2019}\\
%&&&&&\\
\hline
{\bf Galaxy evolution} (\S\ref{sec:gf})&&&&&\\
\hline
$\eta_{\rm feedback}$ & 50-100\% & 3\% & 2\% & kSZ + tSZ + DESI &\cite{battaglia/etal:2019}\\
$p_{\rm nt}$  & 50-100\% & 8\% & 5\% & kSZ + tSZ + DESI & \cite{battaglia/etal:2019}\\
%&&&&&\\
\hline
{\bf Reionization } (\S\ref{sec:reion})&&&&&\\
\hline
$\Delta z$ & 1.4 & 0.4 & 0.3 & TT (kSZ) & \cite{alvarez/etal:2019}\\
\hline
\hline
\end{tabular}
\begin{tablenotes}
\item \textsuperscript{a} Projected 1$\sigma$ errors as in \cite{so_forecast:2019}, with the addition of neutrino mass limits for an optical depth measurement of $\sigma(\tau)=0.002$, achievable with LiteBIRD. 
 Sec. 2 of \cite{so_forecast:2019} describes the methods used to account for noise properties and foreground uncertainties. %Instrumental noise uses a model that reproduces Chile-based CMB performance, with 
 A 20\% end-to-end observation efficiency is used, matching what has been typically achieved in Chile. 
 We assume SO is combined with {\it Planck} data.
\item \textsuperscript{b} 
Primarily from \cite{bk:2018} and \cite{planck_cosmology:2018}. We anticipate data from existing ground-based data
%, including ACT, SPT, Simons Array, CLASS and BICEP/Keck, 
to improve on the `current' limits by 2022. Constraints 
%on these parameters 
are expected to lie between the `current' and SO-Nominal levels.
%\item \textsuperscript{c} 
%The two noise levels, Baseline and Goal, are described in Table 1 and 2 of \cite{so_forecast:2019}. Following \cite{so_forecast:2019}, we increase just the Baseline projected uncertainties by 25\% as a proxy for systematic errors. 
\item \textsuperscript{d} 
The SO observables and external datasets used, as summarized in \cite{so_forecast:2019} except for `LB': LiteBIRD data. 
\item \textsuperscript{e} The SO-Goal projected uncertainty with zero foregrounds is %more than a factor of two smaller: 
$\sigma(r)=0.0007$.
\item \textsuperscript{f} 
Neglecting foreground uncertainties and possible systematic errors, $\sigma(\mnu)$ would be $0.016$~eV for this case. 
\end{tablenotes}
\label{tab:goals}
\end{table*}

%

%tablecomments{
%All of our SO forecasts assume that SO is combined with {\it Planck} data.
%\item \textsuperscript{b} 
%This column reports forecasts from earlier sections (in some cases using 2 s.f.) and applies no additional systematic error.
%\item \textsuperscript{c} 
%This is the nominal forecast, increases the column (a) uncertainties by 25\% as a proxy for instrument systematics, and rounds up to 1 s.f. 
%\item \textsuperscript{d} 
%This is the goal forecast, has negligible additional systematic uncertainties, and rounds to 1 s.f. 
%\item \textsuperscript{e} 
%Primarily from bkp and planck2018_parameters.}

\vspace{-.2in}
\subsection{Primordial perturbations \label{sec:primordial}}
SO targets a refined theory for the early universe by searching for as-yet undetected primordial tensor perturbations, and better characterizing the subtleties of the primordial scalar perturbations.


 \begin{figure}[t!]
%\includegraphics[width=\columnwidth]{figs/fig41a.pdf}
\centering
\includegraphics[width=0.48\columnwidth]{figs/ns_r_v3.pdf}
\includegraphics[width=0.48\columnwidth]{figs/neff_mnu.pdf}
\caption{\small {\bf Left, SO projections (68\% and 95\% limits) for primordial power spectrum parameters :} $n_s$ (the scalar spectral index) and $r$ (the tensor-to-scalar ratio) for vanishingly small tensor modes, compared to current constraints. SO-Nominal is described in  Sec. \ref{sec:science}; SO-Enhanced in Sec \ref{sec:enhance-subsec}. We expect at least a 3$\sigma$ measurement of primordial gravitational waves if $r \ge 0.01$, improving by a factor of 2 with the enhanced SO configuration. {\bf Right, SO projections for neutrino physics (68\% limits):} the total mass of neutrino particles ($\mnu$) and the effective number of relativistic species (\neff). SO should give a clear indication of a non-zero mass sum in the inverted hierarchy (where $\mnu\ge0.1$~eV), and should measure the minimal normal hierarchy at $3-4\sigma$ when combined with LiteBIRD ($\mnu\ge0.06$~eV, indicated).}
\label{fig:pert}
\end{figure}

\noindent
{\bf (a) Tensor-to-scalar ratio, $r$} \cite[SWP][]{shandera/etal:2019}: With its SATs, SO aims to measure $r$ with $\sigma(r)=0.003~(0.002)$ for an $r=0$ model (Fig.~\ref{fig:pert}). %, or $\sigma(r)=0.00$\red{XX} if $r=0.01$. 
 This will enable at least a $3\sigma$ measurement of primordial gravitational waves if $r \ge 0.01$.
%, providing an important test of inflationary models, 
Otherwise, SO will lower the current limit 
%($r<0.06$ at 95\% CL) 
by an order of magnitude.\\
%This constraint will come from the large-scale $B$-modes measured by the SO SATs. \\
 \noindent 
{\bf (b) Scalar perturbations} \cite[SWP][]{slosar/etal:2019b}: Using the CMB power spectra measured by the LAT, SO will halve the current uncertainty on the spectral index of primordial perturbations (to $\sigma(n_s)=0.002$), and aims to estimate the scalar amplitude at the half-percent level at $k=0.2$/Mpc scales. This will test the almost-scale-invariant prediction of inflation over a wider range of scales than  accessible to {\it Planck}.
%, and identify possible deviations from a power law that are characteristic of some alternative models for the early universe. 
%This constraint will come from the small-scale primary CMB power spectra measured by the SO LAT.
\\
 {\bf (c) Non-Gaussianity of perturbations} \cite[SWP][]{meerburg/etal:2019}: SO will constrain $\sigma(f^{\rm local}_{\rm NL})= 2~(1)$, more than halving current constraints.  This will be derived via either the kinematic Sunyaev--Zel'dovich effect, or the CMB lensing field, each correlated with the LSST galaxy distribution, and from the bispectrum, which will also improve constraints on other  non-Gaussianity parameters.\\


%\begin{figure}[t!]
%\includegraphics[width=\columnwidth]{figs/neutrino.pdf}
%\caption{
%Summary of current limits on the neutrino mass scale, $\Sigma m_\nu$, and forecast sensitivity, from cosmological probes and laboratory searches. The mass sum is shown as a function of the mass of the lightest neutrino eigenstate, $m_\mathrm{light}$, for the normal and inverted hierarchy. Current cosmological bounds (TT,TE,EE+lowE+lensing+BAO,~\citealp{planck2018:parameters}) exclude at 95\% confidence the region above the horizontal brown dashed line. The $1\sigma$ sensitivity for \so{} (baseline with no systematic error or goal) combined with large scale structure measurements (LSS, as described in Table~\ref{tab:goals}) is shown for two example cases, enabling a ~$3\sigma$ measurement of $\Sigma m_\nu$ for the minimal mass scenario for the inverted ordering. The expected sensitivity from the $\beta$-decay experiment KATRIN~\cite{Angrik:2005ep} is indicated with a vertical yellow band on the right -- the projection here is done for NH, IH yields similar results with differences not visible on these scales.\\}
%\label{fig:nu}
%\end{figure}

\vspace{-.4in}
\subsection{Effective number of relativistic species\label{sec:Neff} \cite[SWP][]{green/etal:2019}}
A universe with three neutrino species -- and no additional light species -- provides $3.046$ effective relativistic species. SO aims to measure $\sigma(N_{\rm eff})=0.07~(0.05)$, more than halving the current limit from the \planck\ satellite (Fig.~\ref{fig:pert}).
%using the primary CMB temperature and polarization power spectrum measured from the SO LAT, more than halving the current limit from the \planck\ satellite (Fig.~\ref{fig:pert}). 
$\Delta N_{\rm eff} \ge 0.047$ is predicted for models containing additional light non-scalar particles that were in thermal equilibrium with the particles of the Standard Model at any point back to the time of reheating.% SO's target would exclude at more than 95\% confidence any models with three or more such additional particles.
\\

\vspace{-.4in}
\noindent
\subsection{Neutrino Mass \label{sec:mnu}  \cite[SWP][]{dvorkin/etal:2019}}
Within the normal neutrino hierarchy the total mass in the three neutrino species has $\mnu \ge 0.06$~eV, or $\ge 0.1$~eV in the inverted hierarchy. SO aims to measure this total mass with  $\sigma(\mnu)=0.04~(0.03)$~eV (Fig. \ref{fig:pert}), which could give a clear indication of a non-zero mass sum in the inverted hierarchy. SO will use three complementary methods: (i) CMB lensing combined with BAO measurements from DESI; (ii) SZ cluster counts calibrated with weak lensing measurements from LSST; and (iii) thermal SZ distortion maps combined with BAO measurements from DESI. The legacy SO dataset can be combined with LiteBIRD's future cosmic variance-limited measurement of the optical depth to reionization to reach $\sigma(\mnu)$=0.02~eV, which would enable at least a 3$\sigma$ (5$\sigma$) measurement of the mass within the normal (inverted) hierarchy.\\
%, or a $5\sigma$ detection for the inverted hierarchy.\\
  
 
%\begin{figure}[t!]
%\includegraphics[width=\columnwidth]{figs/sz.pdf}
%\caption{Galaxy evolution and reionization.\\}
%\label{fig:sz}
%\end{figure}
 
 \vspace{-.2in}
\subsection{Physics beyond the Standard Cosmological Model\label{sec:de}}
Upcoming optical data promise to constrain deviations from a cosmological constant at redshifts $z<1$. SO will be complementary by measuring the amplitude of matter perturbations, $\sigma_8$, out to $z=4$ with a 2\% constraint between $z=\textrm{1--2}$, and will use the kSZ effect to enable novel tests of modified gravity theories \cite[SWP][]{slosar/etal:2019}. The matter perturbation amplitude will be obtained using SZ galaxy clusters calibrated with LSST weak lensing measurements or SO's own lensing measurements, or using CMB lensing maps cross-correlated with the LSST galaxy number density. SO's lensing measurements will also independently calibrate LSST's multiplicative bias. % At higher redshifts, this will be particularly useful.

SO's precision measurement of the %temperature and polarization 
primordial power spectra will also enable searches for Dark Matter interactions \cite[SWP][]{gluscevic/etal:2019}, constraints on ultra-light axions \cite[SWP][]{grin/etal:2019},  isocurvature perturbations, cosmic strings, and precision tests of Big Bang Nucleosynthesis \cite[SWP][{grohs/etal:2019}. SO will make the most precise measurement to date of birefringence and primordial magnetic fields. 

In looking beyond the known extensions to $\Lambda$CDM, SO will reduce the current uncertainty on the Hubble constant derived from the primary CMB within the \LCDM\ model, reaching a third-percent measurement on $H_0$. In doing so SO will make independent determinations of cosmological parameters using the polarization spectra (EE and TE) instead of intensity (TT), with different foregrounds and systematic effects. A persistent discrepancy in $H_0$ values inferred from the CMB versus Hubble diagram measurements at low redshift \cite[SWP][]{beaton/etal:2019} might indicate new physics.\\

\vspace{-.2in}
\subsection{ Galaxy evolution: feedback efficiency and non-thermal pressure in massive halos  \cite[SWP][]{battaglia/etal:2019,mantz/etal:2019}
\label{sec:gf}}
By measuring the thermal and kinematic Sunyaev--Zel'dovich effects in massive halos, using galaxy positions measured by the DESI spectroscopic survey, SO will inform and refine models of galaxy evolution. %In combination with the DESI spectroscopic survey, 
It will constrain the feedback efficiency in massive galaxies, groups, and clusters, $\eta_{\rm feedback}$, to 3\% (2\%) uncertainty, and the degree of non-thermal pressure support, $p_{\rm nt}$, to 8\% (5\%) uncertainty. No direct constraints on these important galaxy formation parameters have yet been derived from statistically meaningful galaxy samples. %These constraints will be derived from the LAT temperature maps, combined with galaxy positions measured by the DESI spectroscopic survey.
\\

\vspace{-.3in}
\subsection{ Reionization: measurement of duration  \cite[SWP][]{alvarez/etal:2019}\label{sec:reion}}
The reionization process is still poorly characterized. If the duration of reionization $\Delta z > 1$, SO will measure the average duration of reionization with a significance between $2\sigma$ and $3\sigma$, and probe the degree of patchiness of the process, thus constraining models for the ionizing process. Such a measurement would be among the first to probe the properties of the first galaxies, quasars, and the intergalactic medium in the reionization epoch. This measurement is derived from the power spectra and four-point functions of the 
%temperature and polarization 
LAT maps,
%\footnote{The forecasts in SO19 use only the power spectrum; these include the 4-point function following \cite{ferraro/smith:2018}.}
since patchy reionization adds excess variance and higher order statistics to the temperature anisotropies through the kinematic SZ effect \cite{ferraro/smith:2018}.\\


\vspace{-.3in}
\subsection{Legacy data products for science from Solar System to Cosmology}
\label{sec:legacy}
  %across multiple redshifts bins to $z < 1$) 
%and
%its measurements of kinematic Sunyaev-Zel'dovich (kSZ) effect, also
%via cross-correlations with DESI, will measure 


%Sensitive microwave observations will also reveal starburst galaxies, transient radio sources, trace the Milky Way's interstellar medium and even be sensitive to planets in our Outer Solar System.

SO will produce its multifrequency maps of the CMB sky for use by the general astronomical community.  Its high level
products will include  component-separated maps of the blackbody CMB temperature and polarization, the Cosmic Infrared Background \cite[SWP][]{kashlinsky/etal:2019}, and  the integrated thermal pressure. Its Galactic synchrotron and dust maps will reveal insights into  
 the Galactic magnetic field \cite[SWP][]{clark/etal:2019}. SO will trace the projected mass distribution with its  160$\sigma$ measurement of
gravitational lensing.
Its measurements of the thermal SZ effect  will measure the integrated electron pressure to $300 \sigma$.
 %across multiple redshifts bins to $z < 1$).

SO will produce  a legacy galaxy cluster catalog of order 20,000 clusters detected via the SZ effect, and a point source catalog of order 10,000 AGN and 10,000 dusty star-forming galaxies \cite[SWP][]{dezotti/etal:2019,dezotti/etal:2019b}. The high resolution maps, in particular, have sufficiently high mapping speed and sky coverage that they can be used to search for transient sources and/or spatially-varying sources such as Planet X and asteroids \cite[SWP][]{holder/etal:2019}.  Indeed, if warranted, the telescope scan pattern can be optimized for such searches.  



When combined with complementary data from LSST, DESI, Euclid,
SPHEREX, eROSITA and WFIRST, SO will trace the evolution of the
large-scale distribution of mass, electron pressure and electron
density. 
In combination with observations from WISE, Planck CIB, and other surveys of the $z=1-2$ universe, LSST's measurements of the large-scale distribution of galaxies will provide a template for the large-scale distribution of matter.  We will use this template to undo the effects of gravitational lensing and increase SO's sensitivity to primordial gravitational waves (see $A_L = 0.3$ forecasts in Table 2).
%For example, 
In cross-correlations with DESI, its kinematic SZ measurements will trace the integrated electron momentum to $190 \sigma$. %{\bf 190 in Table 2!}





%\begin{table*}[ht!]
%\centering
%\caption[]{Methods used for SO forecasts} \small
%\begin{tabular}{c l c}
%\hline
%\hline
% Method & Description & Section  \\
%\hline
%& &\\
%$TT$/$TE$/$EE$ & Temperature and $E$-mode polarization power spectra  %& \ref{sec:highell} \\
%$BB$ & $B$-mode polarization power spectrum & %\ref{sec:bmodes},\ref{sec:lensing}\\
%$\kappa \kappa$ & CMB lensing convergence power spectrum & %\ref{sec:lensing} \\
%3-pt & Bispectrum  & \ref{sec:bispec} \\
%tSZ-N & Cluster catalog  & \ref{sec:sz} \\
%tSZ-N$\times$$\kappa$ & Cluster masses calibrated using CMB lensing & %\ref{sec:lensing},\ref{sec:sz} \\
%tSZ-Y & tSZ Y-distortion map  & \ref{sec:sz} \\
%$TT$ (kSZ) & kSZ effect measured via the temperature power spectrum & %\ref{sec:highell} \\
%&\\
%\hline
%&\\
%ext delens & Delensing field estimated from large-scale structure %surveys& \ref{sec:bmodes},\ref{sec:lensing} \\
%tSZ-N$\times$LSST-WL & Cluster masses calibrated using LSST weak %lensing data & \ref{sec:sz} \\
%$\kappa \kappa$$\times$LSST-LSS & CMB lensing correlated with galaxy %density in tomographic slices from 3 years of LSST & %\ref{sec:methods},\ref{sec:lensing} \\
%DESI-BAO & BAO measurements from the full DESI survey & %\ref{sec:methods} \\
%DESI & Galaxy positions from the full DESI survey & \ref{sec:sz} \\
%&\\
%\hline
%\hline
%\\
%\end{tabular}
%\label{tab:method}
%\end{table*}




==> table_old.tex <==

\begin{table*}[ht!]
\centering
\caption[Simons Observatory Surveys]{Summary of SO key science goals (numbers to be rounded) \tablenotemark{a}} \small
\begin{tabular}{ l |c| c  c| cc|l}
\hline
\hline
  & Current\tablenotemark{b} & \multicolumn{2}{|c}{ SO-Nominal (2022-27)} & \multicolumn{2}{|c|}{ SO-Enhanced
  (2022-32)\tablenotemark{e}}& \\
    &  & Baseline\tablenotemark{c} & Goal\tablenotemark{d} & Baseline & Goal & Method \\
%&&2022-27&2022-27&2022-32&2022-32&\\
\hline
\hline
{\bf Primordial }   &&&&&&\\
{\bf  perturbations} (\S\ref{sec:primordial})  &&&&&&\\
\hline
$r$ ($A_L=0.5$) & $0.03$ & ${\bf 0.003}$ & $0.002$ & $0.0014$ & $0.0012$ & BB + ext delens \\
$r$ ($A_L=0.3$) &  &  & & $0.0011$ & $0.0009$ & BB + opt delens \\
&&&&&&\\
$n_s$ & 0.004 & 0.002 & {\red{(EC)}} & {\red{(EC)}} & {\red{(EC)}} &TT/TE/EE\\
 $e^{-2\tau}\mathcal{P}(k=0.2 \rm{/Mpc})$ & 3\% & ${\bf 0.5}$\% & 0.4\% & {\red{(RH)}} & {\red{(RH)}} & TT/TE/EE\\
$f^{\rm local}_{\rm{NL}}$&  5& ${\bf 3}$ & 1 & 1  &  1 & $\kappa \kappa$ $\times$ LSST-LSS + 3-pt \\
&& ${\bf 2}$ & 1 &1 & 1 & kSZ + LSST-LSS \\
&&&&&\\
\hline
{\bf Relativistic species} (\S\ref{sec:Neff}) &&&&&&\\
\hline
\neff\ &  0.2 & ${\bf 0.07}$ & 0.05 & 0.05 & {\red{(EC)}} & TT/TE/EE + $\kappa \kappa$\\
&&&&&&\\
\hline
{\bf Neutrino mass} (\S\ref{sec:mnu})&&&&&&\\
\hline
$\mnu$ (eV, $\sigma(\tau)=0.01$) & 0.1 &  ${\bf 0.04}$ & 0.03 & 0.030 & {\red{(MM)}}& $\kappa \kappa$ + DESI-BAO \\
&& ${\bf 0.04}$ & 0.03 & $0.026$ & $0.025$ & tSZ-N $\times$ LSST-WL \\
&& ${\bf 0.05}$ & 0.04 &$0.036$ &$0.035$& tSZ-Y + DESI-BAO \\
&&&&&&\\
$\mnu$ (eV, $\sigma(\tau)=0.002$) & &   $0.021$  & {\red{(MM)}} & {\red{(MM)}}&  {\red{(MM)}}  & $\kappa \kappa$ + DESI-BAO \\
 & &   ${0.019}$  & $0.017$ & $0.016$ &   $0.014$ &  tSZ-N $\times$ LSST-WL \\
 & &   ${0.028}$  & $0.027$ & $0.028$ &   $0.027$ &  tSZ-Y + DESI-BAO \\
&&&&&&\\
\hline
{\bf Beyond standard model}(\S\ref{sec:de}) &&&&&&\\
\hline
$\sigma_8(z=1-2)$& 7\%& ${\bf 2}$\% & 1\% & 0.9\% & 0.7\% &$\kappa \kappa$ + LSST-LSS \\
&& ${\bf 2}$\% & 1\% &{\red{(NB)}}&{\red{(NB)}} & tSZ-N $\times$ LSST-WL \\
$H_0$ ($\Lambda$CDM) & 0.5 &  ${\bf 0.4}$ & 0.3 & {\red{(EC)}} &{\red{(EC)}}& TT/TE/EE + $\kappa \kappa$ \\
&&&&&&\\
\hline
{\bf Galaxy evolution}(\S\ref{sec:gf})&&&&&&\\
\hline
$\eta_{\rm feedback}$ & 50-100\% & ${\bf 3}$\% & 2\%& 2\% & {\red{1\%}}& kSZ + tSZ + DESI \\
$p_{\rm nt}$  & 50-100\% & ${\bf 8}$\% & 5\% &4\% &{\red {3\%}}& kSZ + tSZ + DESI \\
&&&&&&\\
\hline
{\bf Reionization }(\S\ref{sec:reion})&&&&&&\\
\hline
$\Delta z$ & 1.4 &{\red{${\bf 0.6}$}} & {\red {0.3}} & {\red{(MA)}}&{\red{(MA)}}& TT (kSZ 4pt + 2pt) \\
\hline
\hline
\end{tabular}
\begin{tablenotes}
\item \textsuperscript{a} As described in \cite{so_forecast:2019} we calculate instrumental noise using a model that reproduces the  Chile-based AdvACT performance, and we use a 20\% end-to-end observation efficiency that has been typically achieved by Chile-based CMB experiments.  
\item \textsuperscript{a} The flowdown of these science goals to instrument requirements are described in Sec \ref{sec:} of \citet{so_forecast:2019}. All SO forecasts assume that SO is combined with {\it Planck} data.
\item \textsuperscript{b} 
These are primarily from \citealp{bk:2018} and \citealp{planck_cosmology:2018}. We anticipate data from existing ground-based data, including ACT, SPT, Simons Array and BICEP/Keck, to improve on the `current' limits by 2022. Constraints on all these parameters are expected to lie between the reported `current' and the SO-Nominal levels.
\item \textsuperscript{c} 
Nominal forecast, which increases the forecast uncertainties by 25\% as a proxy for instrument systematics, and rounds up to 1 s.f. 
\item \textsuperscript{d} 
Goal forecast, with negligible additional systematic uncertainties, and rounds to 1 s.f. 
\item \textsuperscript{e} 
{\it This is currently the enhanced forecast (3 extra SATs for 5 extra years,  plus fill out the LAT for 5 extra years) with negligible additional systematic uncertainties. KA: make clear where LiteBIRD is included or not}


\end{tablenotes}
\label{tab:goals}
\end{table*}
